It Takes Two to Tango: Towards Theory of AI's Mind

Theory of Mind is the ability to attribute mental states (beliefs, intents, knowledge, perspectives, etc.) to others and recognize that these mental states may differ from one's own. Theory of Mind is critical to effective communication and to teams demonstrating higher collective performance. To effectively leverage the progress in Artificial Intelligence (AI) to make our lives more productive, it is important for humans and AI to work well together in a team. Traditionally, there has been much emphasis on research to make AI more accurate, and (to a lesser extent) on having it better understand human intentions, tendencies, beliefs, and contexts. The latter involves making AI more human-like and having it develop a theory of our minds. In this work, we argue that for human-AI teams to be effective, humans must also develop a theory of AI's mind (ToAIM) - get to know its strengths, weaknesses, beliefs, and quirks. We instantiate these ideas within the domain of Visual Question Answering (VQA). We find that using just a few examples (50), lay people can be trained to better predict responses and oncoming failures of a complex VQA model. We further evaluate the role existing explanation (or interpretability) modalities play in helping humans build ToAIM. Explainable AI has received considerable scientific and popular attention in recent times. Surprisingly, we find that having access to the model's internal states - its confidence in its top-k predictions, explicit or implicit attention maps which highlight regions in the image (and words in the question) the model is looking at (and listening to) while answering a question about an image - do not help people better predict its behavior.

==> source/frogs.tex <==
\section{FROGS}
\begin{enumerate}
%\item Why should the vision community care about this direction? (Motivation) 
%\item take home messages
%\item How does model complexity (parameters, depth, representation power of the function) correlate with a human's ability to assess the machine? 
%\item Elaborate why VQA is a good benchmark to evaluate human-machine collaboration? What collaborative skills does it test? 
%\item Elaborate more on applications. For example, does it help in making strenuous data annotation simpler?
%\item Can you build a model the parameters collected in the survey to estimate how good a human would be at estimating the ability of a robot ? Moreover, do humans who are good at inter-human relationships / team work good at collaborating with AI?
%\item Authors should make a more thorough evaluation with relevant analysis and connections to cognitive theory, human-robot interaction.
%\item Convincing reviewers that this is a problem that people working not only in AI but in vision NEED to thinking about is going to be the primary obstacle.
%\item Refine intro language so that it is easier for the reader to understand. It looks pretty easy to be completely lost on the idea of what theory of mind was after reading the title, abstract, and first few paragraph of the intro. 
%\item Do the results of the analyses generalize to other tasks? In the sense, is there any basis to believe that the trends/conclusions will hold true for other tasks?
%(I see 2 ways of resolving this : if we put this forward as a potential research direction then this is not much of a problem (maybe?), or if we push towards generalizing this, then we need to make a convincing argument)
\item 
\end{enumerate}


==> source/future_work.tex <==
\section{Future Work}
-- Evaluating to what extent this makes a more effective human-AI team for the purpose of accomplishing a specific goal is part of future work. \newline 
% -- "well what does this tell us about how we should move forward"

==> source/meeting_notes.tex <==
\section{Meeting notes, Todos}
\subsection{Feb 10}
Different QI pairs for failure prediction vs. answer prediction. So completely different tasks?
\par 
\subsection{Feb 8}
% * <prabhuviraj@gmail.com> 2017-03-24T23:30:49.111Z:
% ^.
\textbf{High-level:} \newline  
-- Do explanation modalities help people get to know a machine better? Make the machine more predictable: in terms of its successes and failures, and in terms of its responses. At test time, show XAI visualization, or not at test time just during training? Then need separate train and test phase, so don't do that. \newline 
Individual image vs. collage. Train and test. \newline 
Training show feedback. They still guess. At test time, no feedback. So can track accuracies while training also. \newline 
Sort 15 questions bas	ed on image-independent difficulty / likelihood of success. May not be able to do this if workers not trained on all. \par 

Three capabilities:
Failure predictions
Strengths weaknesses (?)
What is it going to say?
\par 
Per question HIT?
\par 
Why VQA? Motivate in paper.
Why these three capabilities? Motivate in paper.
\par 
Decisions:
-- Fixed set of questions. N. Depends budget. Just 15. 
-- For strengths and weaknesses, just these 15. May not be able to do this.
-- Separate train (with feedback) and test phase.
\par 
XAI:
\begin{compactenum}
\item None
\item Confidence
\item Predicted answer distribution
\item Grad-CAM
\item HieCoAtt image
\item HieCoAtt question
\item HieCoAtt image + question
\end{compactenum}
Also check show only at test time and not training. Three settings: nothing, only at test time, during both training and testing. 
\par 
These questions are not important. Why these questions? Call then 15 tasks, not questions. 
\subsection{Feb 17}
\textbf{Note:} Eventually we want AI experts, VQA experts, etc. to do these tasks. 
\subsection{Thoughts based on AC meeting conversation}
Start with the games (bigger images, etc.) or some application where becomes crystal clear why need ToAIM. Maybe play the game or walk through scenario ignoring AI’s quirks, and show how completely fail. Motivate from there. At least in talk. Not sure about paper. \par 

Use motivation from Alert. Why want to predict failure. Know when to use it, when not to use it, etc. Motivations from specification sheet (Aayush’s ECCV 2014 paper). \par 

One future application can be teaching the machine. If I know its current mental state, can better cater future training/curriculum to it. What I am talking about now involves humans approximating decision boundary of AI / neural net. This future training thing involves no just that, but also estimating how SGD will update the decision boundary! So definitely a v2.0 v3.0 thing. But starting from v1.0. Just estimate decision boundary for now: success, failure, predicting output. \par 

One real application can be search. You start with a caption, it asks you questions to know better what exactly you’d like. Like V20Q (Arijit). For visually impaired, application is knowing when to trust and when not to trust. Even for sighted, if I know this agent is good at bird species but not tree species, I’d know when to use it. All the Alert, specification sheet, etc. motivation (again).

==> source/old_intro.tex <==
\section{Introduction}

% Teaser
\begin{figure}[t!]
\setlength{\fboxsep}{0pt}
\setlength{\fboxrule}{0pt}
	\begin{subfigure}[t]{3.5in}	\fbox{\includegraphics[width=3.5in]{figures/teaser_today.png}}
		\caption{Focus of research today}
        \label{fig:fp}
	\end{subfigure}
	\begin{subfigure}[t]{3.5in}
    	%\hspace{0.75in}
		\fbox{\includegraphics[width=3.5in]{figures/teaser_proposed.png}}
		\caption{Proposed research focus}
        \label{fig:kp}
	\end{subfigure}
\caption{(a) Research today -- In human-AI collaborative teams, the burden is on the AI to develop a theory of a human's mind. They predict human behavior, actions, responses, etc. (b) Proposed research agenda -- in addition to AI, the emphasis should also be on humans to build an accurate theory of an AI's mind. \pc{Should we have another teaser figure that actually depicts a particular vision application? Maybe understanding failure modes of VQA. This way, when we talk about the VQA as our domain of experiments either in the introduction or in any subsequent section, we can reference this figure and the associated application.}
}
\end{figure}
Recent studies~\cite{engel2014reading, woolley2010evidence} have looked at why some teams work smarter -- demonstrate more collective intelligence -- than others. Some teams were working remotely and collaborating online, while others were co-located, working face to face. The study found that the most important ingredients for a smart team remained the same irrespective of the mode of interaction: teams with members who communicated a lot, participated equally, and possessed good emotion-reading skills were more effective. The latter refers to the ability to consider and keep track of what other team members feel, know, and believe. In other words, members who demonstrated good Theory of Mind abilities, demonstrated larger collective intelligence.
\par 
% FP, KP interfaces
\begin{figure*}[!t]
\setlength{\fboxsep}{0pt}
\setlength{\fboxrule}{0pt}
	\begin{subfigure}[t]{4in}	\fbox{\includegraphics[width=3.5in]{figures/image15.png}}
		\caption{Snapshot of the Failure prediction interface.}
        \label{fig:fp}
	\end{subfigure}
	\begin{subfigure}[t]{3in}
    	%\hspace{0.75in}
		\fbox{\includegraphics[width=3in]{figures/kp_interface.png}}
      	\hspace{0.75in}
		\caption{Snapshot of the Knowledge prediction interface.}
        \label{fig:kp}
	\end{subfigure}
\caption{(a) A person guesses if an AI agent (Vicki) answered this question for this image correctly or wrongly. (b) A person guesses the exact answer by an AI agent (Vicki) for this question for this image.
}
\end{figure*}

Theory of Mind is ``the ability to attribute mental states -- beliefs, intents, desires, knowledge, etc. -- to oneself and others''. It is the ability ``to understand that others have beliefs, desires, intentions, and perspectives that are different from one's own.''\footnote{\url{https://en.wikipedia.org/wiki/Theory_of_mind}}
\par 

Effective communication involves considering a \new{teammate's background knowledge, abilities, preferences and modify ones interactions accordingly~\cite{grosz2012question}.} Without well developed theory of mind skills, conversations would be disjointed or repetitive, teams would be ineffective.
\par 
As Artificial Intelligence (AI) progresses, we find ourselves working with AI increasingly often to make our lives more productive and convenient. This can be best accomplished if we can form effective teams with AI. 
\par 

Research in AI has placed much of the burden on the AI to play its part in the team: \new{be more accurate~\cite{he2016deep,redmon2016you,szegedy2016inception,ren2015faster,liu2016ssd}, more human-like~\cite{}, understand our intentions~\cite{oliver2000bayesian, vondrick2016predicting, vondrick2016anticipating}, beliefs~\cite{eysenbach2016mistaken}, tendencies~\cite{dubey2015makes}, contexts~\cite{recasens2015they}, and mental states~\cite{}}. In this work, we argue that for human-AI teams to be effective, theory of mind must go both ways. It is equally important for us to understand the AI's beliefs, knowledge, and quirks (tendencies).
\par 
We study this within the scope of a Visual Question Answering (VQA) task where an AI (call it Vicki) is trained to answer free-form natural language questions about images. VQA is a challenging, goal-driven multi-modal task that is applicable to scenarios involving active elicitation of visual information~\cite{antol2015vqa,malinowski2014multi,tu2014joint,bigham2010vizwiz,gao2015you}. We start by assessing the extent to which people can build a theory of AI's mind. \new{To familiarize the human with Vicki, we then train a subject (human) using a number of different explanation modalities such as Vicky's confidence of prediction, image attention maps, question attention maps, their combination~\cite{lu2016hierarchical}, and GradCam visualizations~\cite{selvaraju2016grad}.} Through the entire
process, the human is learning, but Vicki is pre-trained and
fixed. Finally, we test the humans' (shallow and deep) understanding of Vicky via the following tasks: 
\begin{compactenum}
\item Failure prediction (shallow understanding) -- the human guesses whether Vicky will succeed or fail in answering a given question about an image.
\item Knowledge prediction (deep understanding) -- human guesses Vicki's exact response (answer) to a question.
\end{compactenum}
A human's accuracy at these tasks helps operationalize measuring the extent to which the human has built an accurate model of Vicki's ``mental'' state. \new{Through the entire process, the human is learning, but Vicki is pre-trained and fixed.}
\par \noindent
\new{\textbf{Applications.} In cases where humans and AI collaborate together to achieve a goal, a knowledge of the AI's failure modes would help the human account for inaccurate predictions. For instance, if an AI in a self-driving car is unlikely to be able to accurately detect lane markings in an image due to bad lighting conditions, a human who understands the failure modes and behavior of the AI can choose to ignore the unreliable detections for such inputs.} % Applications for failure prediction from ``Alert'', ``Semantic characterizing of failure modes''. Applications for KP -- Visual 20Q?} \par 
% \new{(Emphasize novelty of our project).} 
\par \noindent
\textbf{Contributions:} The contributions of this work are:
\begin{compactenum}
\item Initiating a research agenda around humans building a theory of AI's mind.
\item Operationalizing this agenda in a specific domain of Visual Question Answering (VQA).
\item Studying the effectiveness of different explanation modalities in familiarizing the human with Vicki's strengths and weaknesses.
% DP: Integrate with 2. 
% \item Proposing three tasks that will serve as training tools to help a human get to know Vicki better, and as an evaluation platform to measure how accurate the human's model of Vicki is.
\end{compactenum}
\par 
\new{The remainder of the paper is organized as follows: we first introduce relevant prior art and briefly explain their relation to our work. Following that, we describe the specific AI agent (Vicki) that we use in our experiments. We then present an analysis of people's perception of AI before they are introduced to Vicki. Next, we describe the tasks via which we evaluate a person's understanding of Vicki. We then describe the different ``aids'' that we show people to help them understand Vicki better, and analyze their effectiveness in different settings. Finally, we discuss the implications of this work and possible extensions.}

==> source/perf_analysis.tex <==
\section{Subject Performance Analysis}
\par
In this section, we present further analysis of subject performance on the Failure Prediction (FP) and Knowledge Prediction (KP) tasks. On FP, always
answering “correctly” would result in an accuracy of
58.29\%. Recall that subjects did slightly better and achieved 60\% accuracy on FP, even without prior familiarity with Vicki (No Train).  Thus, subjects are already slightly better calibrated with an AI's capabilities than unbridled optimism (or pessimism). Further recall that after being familiarized via Instant Feedback (IF), subjects perform signficantly better than the No Train setting, achieving 13.1\% higher mean accuracies.
\par

In KP, answering each question with Vicki's most popular answer overall (`no') would lead to an accuracy of 13.4\%.
Additionally, answering each question with Vicki's most popular answer \emph{for that question}\footnote{Vicki's most frequent answer (in the train set) to each question is as follows: What kind of animal is this? (Dog) What time is it? (Daytime). What are the people doing? (Standing) Is it raining? (No) What room is this? (Kitchen) How many people are there? (1) What color is the umbrella? (Black) } leads to an accuracy of 31.4\%. Interestingly, humans subjects who are unfamiliar with Vicki (No Train) achieve 24.8\% accuracy -- better than the most popular answer overall prior, but worse than the question-specific prior over Vicki's answers. The latter is understandable as subjects unfamiliar with Vicki do not know which of its 1000 possible answers are more likely a priori for each question. However, humans subjects who are familiar with Vicki (Instant Feedback setting) considerably outperform both the `most popular answer' and `most popular answer per question' priors, achieving 51.1\% accuracy. It is apparent that just from a few (50) training examples, subjects learn to generalize beyond Vicki's favorites among it's vocabulary of 1000 answers.

==> source/survey_demog.tex <==
\section{Survey Demographics}
We show the population demographics in Fig.~\ref{fig:pop_demog}.
\begin{figure*}[t]
 \centering 
 \includegraphics[width=1\textwidth]{./figures/population_demog.pdf}
 \vspace{-20pt}
 \caption{Population Demographics}
 \vspace{-15pt}
\label{fig:pop_demog}
\end{figure*}
We show the subjects' technology and AI exposure in Fig.~\ref{fig:tech_expo}.
\begin{figure*}[t]
 \centering 
 \includegraphics[width=1\textwidth]{./figures/tech_ai_exposure.pdf}
 \vspace{-20pt}
 \caption{Technology and AI exposure}
 \vspace{-15pt}
\label{fig:tech_expo}
\end{figure*}
We show the perception of AI among the subjects in Fig.~\ref{fig:ai_percep}.
\begin{figure*}
 \centering 
 \includegraphics[width=1\textwidth]{./figures/ai_perception.pdf}
 \vspace{-20pt}
 \caption{Perception of AI}
 \vspace{-15pt}
\label{fig:ai_percep}
\end{figure*}

==> source/survey_ques.tex <==

\section{Survey Questions}
In this section we describe the survey that subjects were asked to answer before carrying out the FP and KP tasks described in Sections 6.1 and 6.2 of the main paper. These questions attempt to assess the subjects' general impressions of present-day AI, and can be broken down into 3 categories -- Population Demographics, Exposure to AI, and Perception of AI. 

As part of the survey, subjects were asked a few subjective questions about their opinions on present--day AI's capabilities. Specifically, they were asked to list tasks that they thought AI is capable of performing \emph{today} (see Fig.~\ref{fig:ai_now}), will be capable of \emph{in the next 3 years} (see Fig.~\ref{fig:ai_3_yrs}), and will be capable of \emph{in the next 10 years} (see Fig.~\ref{fig:ai_10_yrs}). We also asked how \emph{they} think AI works (see Fig.~\ref{fig:how_ai_works}). In Fig.~\ref{fig:ai_now}, ~\ref{fig:ai_3_yrs} and ~\ref{fig:ai_10_yrs}, we show word clouds corresponding to what subjects thought about the capabilities of AI. We also share some of those responses below.

% \newpage
\begin{compactenum}
\item Name three things that you think AI today can do.

\emph{Predict sports games; Detect specific types of cancer in images; Control house temp based on outside weather; translate; calculate probabilities; Predictive Analysis; AI can predict future events that happen like potential car accidents; lip reading; code; Facial recognition; Drive cars; Play Go; predict the weather; Hold a conversation; Be a personal assistant; Speech recognition; search the web quicker.}

\item Name three things that you think AI today can't yet do but will be able to do in 3 years.

\emph{Fly planes; Judge emotion in voices; Predict what I want for dinner; perform surgery; drive cars; manage larger amounts of information at a faster rate; think independently totally; play baseball; drive semi trucks; Be a caregiver; anticipate  a person's lying ability; read minds; Diagnose patients; improve robots to walk straight; Run websites; solve complex problems like climate change issues; program other ai; guess ages; form conclusions based on evidence; act on more complex commands; create art.}

\item Name three things that you think AI today can't yet do and will take a while ($>$ 10 years) before it can do it.

\emph{Imitate humans; be indistinguishable from humans; read minds; Have emotions; Develop feelings; make robots act like humans; truly learn and think; Replace humans; impersonate people; teach; be a human; full AI with personalities; Run governments; be able to match a human entirely; take over the world; Pass a turing test; be a human like friend; intimacy; Recognize things like sarcasm and humor.}
\end{compactenum}

\begin{figure}[t]
 \centering 
 \includegraphics[width=1\linewidth]{./figures/ai_now.png}
 \vspace{-20pt}
 \caption{A word cloud of subject responses to ``Name three things that you think AI today can do.''}
 \vspace{-13pt}
\label{fig:ai_now}
\end{figure}

\begin{figure}[t]
 \centering 
 \includegraphics[width=1\linewidth]{./figures/ai_3_yrs.png}
 \vspace{-20pt}
 \caption{A word cloud of subject responses to ``Name three things that you think AI today can't yet do but will be able to do in 3 years.''}
 \vspace{-13pt}
\label{fig:ai_3_yrs}
\end{figure}

\begin{figure}[t]
 \centering 
 \includegraphics[width=1\linewidth]{./figures/ai_10_yrs.png}
 \vspace{-20pt}
 \caption{A word cloud of subject responses to ``Name three things that you think AI today can't yet do and will take a while ($>$ 10 years) before it can do it.''}
 \vspace{-21pt}
\label{fig:ai_10_yrs}
\end{figure}

Interestingly, we observe a steady progression in subjects' expectations of AI's capabilities, as the time span increases. On a high-level reading through the responses, we notice that subjects believe that AI today can successfully perform tasks such as \emph{machine translation}, \emph{driving vehicles}, \emph{speech recognition}, \emph{analyzing information and drawing conclusions}, etc. (see Fig.~\ref{fig:ai_now}). It is likely that this is influenced by the subjects' exposure to or interaction with some form of AI in their day-to-day lives. When asked about what AI can do three years from now, most subjects suggested more sophisticated tasks such as \emph{inferring emotions from voice tone}, \emph{performing surgery}, and even \emph{dealing with climate change issues} (see Fig.~\ref{fig:ai_3_yrs}). However, the most interesting trends emerge while observing subjects' expectation of what AI can achieve in the next 10 years (see Fig.~\ref{fig:ai_10_yrs}). A major proportion of subjects believe that AI will gain the ability to \emph{understand and emulate human beings}, \emph{teach human beings}, \emph{develop feelings and emotions} and \emph{pass the Turing test}. 

\begin{figure}[t]
 \centering 
 \includegraphics[width=1\linewidth]{./figures/how_ai_works.png}
 \vspace{-20pt}
 \caption{A word cloud of subject responses when asked to describe how \emph{they} think AI today works. 
%  \new{Subjects believe AI is system that has been programmed to perform specific tasks by exposing it to huge amounts of information.}
 }
 \vspace{-23pt}
\label{fig:how_ai_works}
\end{figure}

We also observe how subjects think AI works (see Fig.~\ref{fig:how_ai_works}). Mostly, subjects believe that an AI agent today is a system with high computational capabilities that has been programmed to simulate intelligence  and perform certain tasks by exposing it to huge amounts of information, or, as one of subjects phrased it -- \emph{broadly AI recognizes patterns and creates optimal actions based on those patterns towards some predefined goals}. In summary, it appears that subjects have high expectations from AI, given enough time. While it is uncertain at this stage how many, or how soon, these feats will actually be achieved, we believe that building Theory of AI's mind skills will help humans generally become more active and effective collaborators in human--AI teams. 

We now provide a full list of all questions in the survey. In Fig.~\ref{fig:pop_demog},~\ref{fig:tech_expo} and ~\ref{fig:ai_percep}, we also break down the 321 subjects that completed the survey by their response to each question.

\begin{compactenum}
\item How old are you?
	\begin{compactenum}
	\item Less than 20 years
    \item Between 20 and 40 years
    \item Between 40 and 60 years
    \item Greater than 60 years
	\end{compactenum}
\item What is your gender?
 	\begin{compactenum}
 	\item Male
    \item Female
    \item Other
 	\end{compactenum}
\item Where do you live?
 	\begin{compactenum}
 	\item Rural
 	\item Suburban
 	\item Urban
 	\end{compactenum}
\item Are you?
 	\begin{compactenum}
 	\item A student
 	\item Employed
 	\item Self-employed
 	\item Unemployed
 	\item Retired 
 	\item Other
 	\end{compactenum}
% \newpage
\item To which income group do you belong?
 	\begin{compactenum}
 	\item Less than 5000\$ per year
 	\item 5,000-10,000\$ per year
 	\item 10,000-25,000\$ per year
 	\item 25,000-60,000\$ per year 
 	\item 60,000-120,000\$ per year 
 	\item More than 120,000\$ per year
 	\end{compactenum}
\item What is your highest level of education?
 	\begin{compactenum}
 	\item No formal education
 	\item Middle School
 	\item High School
 	\item College (Bachelors)
 	\item Advanced Degree
 	\end{compactenum}
\item What was your major?
 	\begin{compactenum}
 	\item Computer Science / Computer Engineering
 	\item Engineering but not Computer Science
 	\item Mathematics / Physics
 	\item Philosophy
 	\item Biology / Physiology / Neurosciences
 	\item Psychology / Cognitive Sciences
 	\item Other Sciences
 	\item Liberal Arts
 	\item Other
 	\item None
 	\end{compactenum}
\item Do you know how to program/code?
 	\begin{compactenum}
 	\item Yes
 	\item No
 	\end{compactenum}
\item Does your full-time job involve:
 	\begin{compactenum}
 	\item No computers
 	\item Working with computers but no programming/coding
 	\item Programming/Coding
 	\end{compactenum}
\item How many hours a day do you spend on your computer/laptop/smartphone?
 	\begin{compactenum}
 	\item Less than 1 hour
 	\item 1-5 hours
 	\item 5-10 hours
 	\item Above 10 hours
 	\end{compactenum} 
\item Do you know what Watson is in the context of Jeopardy?
 	\begin{compactenum}
 	\item Yes
 	\item No
 	\end{compactenum}
\newpage
\item Have you ever used Siri, Alexa, or Google Now/Google Assistant?
 	\begin{compactenum}
 	\item Yes
 	\item No
 	\end{compactenum}
\item How often do you use Siri, Alexa, Google Now, Google Assistant, or something equivalent?
 	\begin{compactenum}
 	\item About once every few months
 	\item About once a month
 	\item About once a week
 	\item About 1-3 times a day
 	\item More than 3 times a day
 	\end{compactenum}
% \newpage
\item Have you heard of AlphaGo?
 	\begin{compactenum}
 	\item Yes
 	\item No
 	\end{compactenum}
\item Have you heard of Machine Learning?
 	\begin{compactenum}
 	\item Yes
 	\item No
 	\end{compactenum}
\item Have you heard of Deep Learning?
 	\begin{compactenum}
 	\item Yes
 	\item No
 	\end{compactenum}
\item When did you first hear of Artificial Intelligence (AI)?
	\begin{compactenum}
	\item I have not heard of AI
	\item More than 10 years ago
	\item 5-10 years ago
	\item 3-5 years ago
	\item 1-3 years ago
	\item In the last six months
	\item Last month
	\end{compactenum}
\item How did you learn about AI?
	\begin{compactenum}
	\item School / College
	\item Conversation with people
	\item Movies
	\item Newspapers
	\item Social media
	\item Internet
	\item TV
	\item Other
	\end{compactenum}
\item Do you think AI today can drive cars fully autonomously?
	\begin{compactenum}
	\item Yes
	\item No
	\end{compactenum}
\item Do you think AI today can automatically recognize faces in a photo?
	\begin{compactenum}
	\item Yes
	\item No
	\end{compactenum}
\item Do you think AI today can read your mind?
	\begin{compactenum}
	\item Yes 
	\item No
	\end{compactenum}
\item Do you think AI today can automatically read your handwriting?
	\begin{compactenum}
	\item Yes
	\item No
	\end{compactenum}
\newpage
\item Do you think AI today can write poems, compose music, make paintings?
	\begin{compactenum}
	\item Yes
	\item No
	\end{compactenum}
\item Do you think AI today can read your Tweets, Facebook posts, etc. and figure out if you are having a good day or not?
	\begin{compactenum}
	\item Yes
	\item No
	\end{compactenum}
% \newpage
\item Do you think AI today can take a photo and automatically describe it in a sentence?
	\begin{compactenum}
	\item Yes
	\item No
	\end{compactenum}
\item Other than those mentioned above, name three things that you think AI today can do.
\item Other than those mentioned above, name three things that you think AI today can't yet do but will be able to do in 3 years.
\item Other than those mentioned above, name three things that you think AI today can't yet do and will take a while ($>$ 10 years) before it can do it.
\item Do you have a sense of how AI works?
	\begin{compactenum}
	\item Yes
	\item No
	\item If yes, describe in a sentence or two how AI works.
	\end{compactenum}
\item Would you trust an AI's decisions today?
	\begin{compactenum}
	\item Yes
	\item No
	\end{compactenum}
\item Do you think AI can ever become smarter than the smartest human?
	\begin{compactenum}
	\item Yes
	\item No
	\end{compactenum}
\item If yes, in how many years?
	\begin{compactenum}
	\item Within the next 10 years
	\item Within the next 25 years
	\item Within the next 50 years
	\item Within the next 100 years
	\item In more than 100 years
	\end{compactenum}
\item Are you scared about the consequences of AI?
	\begin{compactenum}
	\item Yes
	\item No
	\item Other
	\item If other, explain.
	\end{compactenum}
\end{compactenum}
\vspace{-5pt}
\begin{figure*}[t]
 \centering 
 \includegraphics[width=1\textwidth]{./figures/population_demog.jpeg}
 \vspace{-20pt}
 \caption{Population Demographics (across 321 subjects)}
 \vspace{-15pt}
\label{fig:pop_demog}
\end{figure*}
\begin{figure*}[t]
 \centering 
 \includegraphics[width=1\textwidth]{./figures/tech_ai_exposure.jpeg}
 \vspace{-20pt}
 \caption{Technology and AI exposure (across 321 subjects)}	
 \vspace{-15pt}
\label{fig:tech_expo}
\end{figure*}
\begin{figure*}
 \centering 
 \includegraphics[width=1\textwidth]{./figures/ai_perception.jpeg}
 \vspace{-20pt}
 \caption{Perception of AI (across 321 subjects)}
 \vspace{-15pt}
\label{fig:ai_percep}
\end{figure*}





